Particle-based Variational Inference with Preconditioned Functional Gradient Flow

Particle-based variational inference (VI) minimizes the KL divergence between model samples and the target posterior with gradient flow estimates. With the popularity of Stein variational gradient descent (SVGD), the focus of particle-based VI algorithms has been on the properties of functions in Reproducing Kernel Hilbert Space (RKHS) to approximate the gradient flow. However, the requirement of RKHS restricts the function class and algorithmic flexibility. This paper offers a general solution to this problem by introducing a functional regularization term that encompasses the RKHS norm as a special case. This allows us to propose a new particle-based VI algorithm called preconditioned functional gradient flow (PFG). Compared to SVGD, PFG has several advantages. It has a larger function class, improved scalability in large particle-size scenarios, better adaptation to ill-conditioned distributions, and provable continuous-time convergence in KL divergence. Additionally, non-linear function classes such as neural networks can be incorporated to estimate the gradient flow. Our theory and experiments demonstrate the effectiveness of the proposed framework.

==> parts/backup.tex <==
\begin{lemma} Under Assumption \ref{}, 

$$
\left|\frac{d^2D_{\mathrm{KL}}(\tilde{p}_{t+s})}{ds^2}\right|
\leq B
\int p_t(x) \left<g(t,x),\nabla\ln\frac{p_*(x)}{p_t(x)}\right>dx
$$
\end{lemma}


\begin{align*}
 g^k_t(x) =&   \int \frac{1}{\sqrt{2\pi|\Sigma_t|}}\exp\left(-
    \frac{1}{2}(y-\mu_t)^\top\Sigma_t^{-1}(y-\mu_t)
    \right)
    \frac{1}{\sqrt{\sigma^2}}\exp\left(-
    \frac{1}{2\sigma^2}\Vert y-x\Vert^2
    \right)\nonumber\\
    &
    \left(\Sigma_*^{-1}(y-\mu_*)-\Sigma_t^{-1}(y-\mu_t)\right)dy\\
    =&\int \frac{1}{\sqrt{2\pi|\Sigma_t|}}\exp\left(-
    \frac{1}{2}\ty^\top\Sigma_t^{-1}\ty
    \right)
    \frac{1}{\sqrt{\sigma^2}}\exp\left(-
    \frac{1}{2\sigma^2}\Vert \ty+\mu_t-x\Vert^2
    \right)\nonumber\\
    &
    \left(\Sigma_*^{-1}(\ty+\mu_t-\mu_*)-\Sigma_t^{-1}\ty\right)d\tilde{y}\\
    =&\int 
    \frac{\sqrt{2\pi |(\sigma^{-2} I + \Sigma^{-1}_t)^{-1}|}}{\sqrt{2\pi \sigma^2|\Sigma_t|}}
    \frac{1}{\sqrt{2\pi |(\sigma^{-2} I + \Sigma^{-1}_t)^{-1}|}}\exp\left(-
    \frac{1}{2}(\ty-\mu_x)^\top\left(\sigma^{-2} I + \Sigma_t^{-1}\right)(\ty-\mu_x)
    \right)\nonumber\\
    &\exp\left(\frac{1}{2}(\mu_t-x)^\top \Sigma_t^{-1} (\mu_t-x)\right)\left(\Sigma_*^{-1}(\ty+\mu_t-\mu_*)-\Sigma_t^{-1}\ty\right)d\tilde{y}\\
    =&\int 
    \frac{1}{\sqrt{ \sigma^2|\Sigma_t(\sigma^{-2} I + \Sigma_t^{-1})|}}
    \tilde{p}(\ty)\exp\left(\frac{1}{2}(\mu_t-x)^\top \Sigma_t^{-1} (\mu_t-x)\right)\left(\Sigma_*^{-1}(\ty+\mu_t-\mu_*)-\Sigma_t^{-1}\ty\right)d\tilde{y}\\
    =& C_x \left(\left(\Sigma_*^{-1}-\Sigma_t^{-1}\right)\mu_x + 
    \Sigma_*^{-1} (\mu_t-\mu_*)
    \right)
\end{align*}
where $$\mu_x = \sigma^{-2}\left(\sigma^{-2} I + \Sigma_t^{-1}\right)^{-1}(x-\mu_t )=\left( I + \sigma^{2}\Sigma_t^{-1}\right)^{-1}(x-\mu_t ),$$ $$C_x = \frac{1}{\sqrt{|\sigma^2 I +\Sigma_t|}}\exp\left(-\frac{1}{2\sigma^2}(x-\mu_t)^\top (I-(I+\sigma^2 \Sigma_t^{-1})^{-1}) (x-\mu_t)\right)$$


\subsection{Proof of Proposition}

\begin{proof}

Consider that $s_\theta(x) = \theta \psi(x)$,

\begin{align}
    \hat{L}(\theta)=\int p_t (\psi(x)^\top\theta^\top\theta\psi(x)+2\operatorname{tr}(\theta\nabla \psi(x)))
\end{align}

\begin{align}
    \frac{d}{d\theta}\hat{L}(\theta)=\int p_t(x) 2 (\theta \psi(x)\psi(x)^\top+\nabla\psi(x)^\top)dx=0
\end{align}

Thus,
\begin{align}
    \theta =\int p_t(y) \nabla \psi(y)^\top dy \left(\int p_t(y) \psi(y)\psi(y)^\top dy\right)^{-1}.
\end{align}

\end{proof}



\begin{algorithm}
\small
\DontPrintSemicolon
\KwInput{training data samples $\{z_i\}_{i=1}^n$, parametric model $p(z|x)=p_x(z):\mathcal Z\rightarrow \RR_+$, prior $p(x)$,
$f_\theta(x):\RR^d\rightarrow\RR^d$, 
$f_0(x):\RR^d\rightarrow\RR^d$
, initial particles (parameters) $\{x^i_0\}_{i=1}^m$, $\theta_0$, 
iteration parameter $T,T',T_0'$, learning rate $\eta,\eta'$, sample size $K$,
}
\For{$t=1,\dots,T$}{
\eIf{$t=1$}
{$T_1 = T_0'$}
{$T_1 = T'$}

Assign $\theta^0_t = \theta_{t-1} $;

\For{$t'=1,\cdots,T_1$}{
Compute unnormalized log-posterior $\log p(x|z_1,\cdots,z_n)$: 
$
U(x) = - \sum_{i=1}^n\log p(x|z_i) - \log p(x)
$

\eIf{Randomized trace estimation}
 {Sample $\{\xi_i\}_{i=1}^K$, such that $\EE\xi=0$ and $\cov \xi = I$;
 
 Compute $\hat{L}(\theta) = \frac{1}{m}\sum_{i=1}^m \left(Q(f_\theta(x_t^i)+f_0(x_t^i)) - f_\theta(x_t^i)\cdot \nabla U(x_t^i) - \frac{1}{K}\sum_{j=1}^K\xi_j^\top \nabla f_\theta(x_t^i) \xi_j\right) $
 }
 {Compute $\hat{L}(\theta) = \frac{1}{m}\sum_{i=1}^m \left( Q(f_\theta(x_t^i)+f_0(x_t^i)) - f_\theta(x_t^i)\cdot \nabla U(x_t^i) - \nabla\cdot f_\theta(x_t^i)\right) $  }
 
 Update $\theta_t^{t'} = \theta_t^{t'-1} - \eta'\nabla \hat{L}(\theta_t^{t'-1})$;
}

Assign $\theta_t = \theta_{t}^{T_1} $;



Update particles
$x^i_t=x^i_t + \eta  \left( f_0(x_t^i) + f_{\theta_t}(x_t^i)\right)$ for all $i=1,\cdots,m$
}

\KwReturn{Optimized particles $\{x^i_T\}_{i=1}^m$}
\caption{Bregman Regularized Stein Variational Gradient}
\end{algorithm}


\begin{algorithm}
\small
\DontPrintSemicolon
\KwInput{training data samples $\{z_i\}_{i=1}^n$, parametric model $p(z|x)=p_x(z):\mathcal Z\rightarrow \RR_+$, prior $p(x)$,
$f_\theta(x):\RR^d\rightarrow\RR^d$, 
%$f_0(x):\RR^d\rightarrow\RR^d$,
 initial particles (parameters) $\{x^i_0\}_{i=1}^m$, $\theta_0$, 
iteration parameter $T,T'$, learning rate $\eta,\eta'$, sample size $K$,
}
\For{$t=1,\dots,T$}{

Assign $\theta^0_t = \theta_{t-1} $;

\For{$t'=1,\cdots,T'$}{
Compute unnormalized log-posterior $\log p(x|z_1,\cdots,z_n)$: 
$
U(x) = - \sum_{i=1}^n\log p(x|z_i) - \log p(x)
$


 {Compute $\hat{L}(\theta) = \frac{1}{m}\sum_{i=1}^m \left( Q(f_\theta(x_t^i)) - f_\theta(x_t^i)\cdot \nabla U(x_t^i) - \nabla\cdot f_\theta(x_t^i)\right) $  }
 
 Update $\theta_t^{t'} = \theta_t^{t'-1} - \eta'\nabla \hat{L}(\theta_t^{t'-1})$;
}

Assign $\theta_t = \theta_{t}^{T_1} $;



Update particles
$x^i_t=x^i_t + \eta  \left(  f_{\theta_t}(x_t^i)\right)$ for all $i=1,\cdots,m$
}

\KwReturn{Optimized particles $\{x^i_T\}_{i=1}^m$}
\caption{Bregman Regularized Stein Variational Gradient}
\end{algorithm}



In fact, we can consider that $k_c(x,y) = (x-c)^\top K (y-c)$.
$$
\begin{aligned}g(t,x)= & \hat{W}_{t}\psi(x)\\
= & \int p(t,y)(-\Sigma_{*}^{-1}(y-\mu_{*})+\Sigma_{t}^{-1}(y-\mu_{t}))(y-c)^{\top}dy\cdot K(x-c)\\
= & -\int p(t,y)(\Sigma_{*}^{-1}(yy^{\top}-\mu_{*}y^{\top}-yc^{\top}+\mu_{*}c^{\top}))dyK(x-c)\\
 & +\int p(t,y)(\Sigma_{t}^{-1}(yy^{\top}-\mu_{t}y^{\top}-yc^{\top}+\mu_{t}c^{\top}))dyK(x-c)\\
= & -\Sigma_{*}^{-1}(\Sigma_{t}+(\mu_{t}-\mu_{*})(\mu_{t}-c)^{\top})K(x-c)\\
 & +\Sigma_{t}^{-1}(\Sigma_{t}-c\mu_{t}^{\top}+\mu_{t}c^{\top}))K(x-c)
\end{aligned}
$$
\begin{align}\label{eq:linear}
 g(t,x) = -\Sigma_{*}^{-1}(\Sigma_{t}+(\mu_{t}-\mu_{*})(\mu_{t}-c)^{\top})K(x-c) +\Sigma_{t}^{-1}(\Sigma_{t}-c\mu_{t}^{\top}+\mu_{t}c^{\top}))K(x-c)
 \end{align}
 
 
 
 \section{More Results}

\subsection{$f_0$}

%In high dimension space, 
%approximate $\nabla\ln\frac{p_*(x)}{p_t(x)}$ is usually difficult, especially for those 
%the function space $\cF$ is usually insufficient






In our previous sections, $f_0(x)$ is a arbitrary base function. In some cases,
the introduction of $f_0$ simplify the learning process of $\nabla\ln \frac{p_*(x)}{p_t(x)}$. %We will discuss. 
In practice, the approximation of $\nabla \ln p_t(x)/p_*(x)$ may not be accurate in general. Thus, we consider two cases: (1) when the variance of $p_0$ is more flat than $p_*$, then we need more 
driving force to make the particle converge; (2) when the variance of $p_0$ is smaller than $p_*$, then we need more repulsive force to make the particle match $p_*$. Since $p_*$ is known, an intuitive way to assign $f_0$ as $\alpha \nabla \ln p_*(x)$, where $\alpha>0$ for case (1);  $\alpha<0$ for case (2). Note that the practical normalization and initialization leads to case (1). 

Intuitively, for case (1), to boost the learning of $\nabla\ln\frac{p_*(x)}{p_t(x)} = \nabla\ln{p_*(x)} - \nabla\ln{p_t(x)} $, $f_0(x)$ takes a part of $\nabla\ln{p_*(x)}$ and makes the learning algorithm to approximate $(1-\alpha)\nabla\ln{p_*(x)} - \nabla\ln{p_t(x)}$. When $\alpha = 1$, the learning objective is equivalent with score matching.

%\begin{proposition} (Score matching) When $f_0(x)=\nabla \ln p_*(x)$, $Q(x) = \frac{1}{2}\Vert x\Vert^2_2$, our algorithm is equivalent with score matching.
%\end{proposition}



Note that when $\cF$ approximates all $\nabla\ln\frac{p_*(x)}{p_t(x)}$ well, the introduction of $f_0(x)$ boosts the learning process but
would not changes the solution of variational gradient. However, when $\cF$ is not large enough, such as linear function class, the introduction of $f_0$ can be recognized as an extension for the function class. We will show an example in Figure \ref{fig:f0}.

\begin{figure}[ht]
    \centering
    \begin{tabular}{cccc}
      \includegraphics[width=0.2\textwidth]{figs/true1k_sample.pdf}  &
  \includegraphics[width=0.2\textwidth]{figs/sample_0_sample.pdf}  
        & \includegraphics[width=0.2\textwidth]{figs/sample_1_sample.pdf}
        & \includegraphics[width=0.2\textwidth]{figs/sample_01_sample.pdf}
\\
{\footnotesize (a) Samples}
&
{\footnotesize (b) $f_0(x)=0$}&
{\footnotesize (c) $f_0(x)=\nabla \ln p_*(x)$}&
{\footnotesize (d) $f_0(x)=\frac{1}{10}\nabla \ln p_*(x)$}
    \end{tabular}
    
   % \includegraphics[width=3.5cm]{figs/graph.png}
   
    \caption{Effect of $f_0$ on linear function class
    for Gaussian mixture
    (10 clusters, $p_0=\mathcal N(0,I)$)
    }%parameterized by $\phi$
    %p_\theta(x,z,u) =
    %induced by $G_\theta^{-1}$
    \label{fig:f0}
\end{figure}

\noindent \textbf{Remark:} When $f_0(x) = \nabla \ln p_*(x)$ and $Q(x) = \frac{1}{2}x^\top x$, the algorithm is equivalent to score matching. In other words, our algorithm can be recognized as a general framework to bridge Stein variational gradient and score matching: When $p(t,x)=p_*(x)$, the optimal $f$ is $0$, we can choose $f_0(x) = \nabla \ln p_*(x)$ and estimate $f_\theta(x) \approx -\nabla \ln p_*(x)$.

==> parts/body.tex <==
\section{Background}


We start with a transportation problem that given $X_0$, we have evolution  equation,  
\begin{equation}\label{eq:transport}
   dX_t = g_t(X_t) . 
\end{equation}


%\begin{align}
%mathcal L(\pi) = \int \log \frac{d\pi}{d\pi_*}d\pi
%\end{align}
Our aim is to sample from $X_t$ such that the distribution of $\pi_t$ should be as close as enough to $\pi_*$. The metric is Kullback-Leibler (KL) divergence by default. 
Note that we focus on the case that $\pi_t$ are smooth distributions with nonzero densities, so that the density function $p_t = {d\pi_t}/{dx}$, $p_* = {d\pi_*}/{dx}$ and the corresponding potential function $U_t(x)=-\log p_t(x)$, $U_*(x)=-\log p_*(x)$ can be well-defined.
\begin{align}
\mathcal L(p) = \int p(x) \log \frac{p(x)}{p_*(x)}dx
\end{align}

By the continuity equation, if $\pi_t$/$p_t$ follows the maximum slope, we have that,
%\begin{align}
%\frac{\partial \pi_t}{\partial t} = -     \nabla\cdot\left(\pi_t \frac{\delta \mathcal F(\pi_t)}{\delta \pi_t}\right)= \nabla\cdot\left(\pi_t \nabla \log\frac{d \pi_*}{d \pi_t}\right)
%\end{align}
\begin{align}
\frac{\partial p_t}{\partial t} = -     \nabla\cdot\left(p_t \frac{\delta \mathcal L(p_t)}{\delta p_t}\right)= \nabla\cdot\left(p_t \nabla \log\frac{ p_*}{ p_t}\right)
\end{align}

Thus, the Wasserstein gradient flow based $g^*_t$ is
\begin{align}\label{eq:grad}
g^*_t(x) = \nabla \log\frac{p_*(x)}{p_t(x)} = \nabla \log p_*(x) - \nabla \log p_t(x)
\end{align}

Although Eq. \eqref{eq:grad} is the exact form of Wasserstein gradient flow, the practical implementation is non-trivial, especially for the entropy gradient $\nabla\log p_t$. Euler–Maruyama method (such as Langevin dynamics; Markov chain Monte Carlo (MCMC)) leverages diffusion to implement the entropy term, but the introduction of stochastic component brings the biased gradient discretization and undetermined transportation map for each particle. Another possibility to implement Wasserstein gradient flow is by kernelization: SVGD maps Wasserstein gradient to reproducing kernel Hilbert space (RKHS), which makes entropy term tractable with kernel divergence. The entropic gradient can be reduced to integral over $p_t$ using an integral by parts. 
Unlike these two strategies, we focus on a parametric approximation of $\log p_t(x)$.
We intend to approximate $\nabla U_t(x)$ with a parametric function $s_\theta(x)$. \citet{hyvarinen2005estimation} mentioned that the estimation of $\nabla U_t(x)$ can be obtained by a closed-form loss function,
\begin{equation}\label{eq:sm}
    L_{\mathrm{SM}}(\theta) = \int p_t(x) \left\Vert s_\theta(x) - \nabla\log p_t(x)\right\Vert^2 dx   
\end{equation}


\begin{proposition}\label{prop:sm} The score matching loss in Eq. \eqref{eq:sm} can be reformulated (with a constant gap) as 
\begin{equation}
 \hat{L}_{\mathrm{SM}}(\theta) = \int p_t(x) \left(\Vert s_\theta(x)\Vert^2 + 2\nabla\cdot s_\theta(x)\right)dx.
\end{equation}

\end{proposition}

With simple derivation, Eq. \eqref{eq:sm} can be rewritten as a tractable form (Proposition \ref{prop:sm}). Then for each step, when we approximate $\nabla\log p_t(x)$ with our parametric function $s_\theta$, 
\begin{equation}
    \theta_t = \argmin_\theta \hat{L}_{\mathrm{SM}} (\theta),
\end{equation}
we have $s_{\theta_t}(x)\approx \nabla \log p_t(x)$. We can update particles as $dX_t = g_t^{\theta_t}(X_t)$, such that
\begin{equation}
    g^{\theta_t}_t(x) = \nabla \log p_*(x) - s_{\theta_t}(x)
\end{equation}

\subsection{Comparison with SVGD}\label{sec:comparison}

In the continuous limit, the SVGD update particles as $dX_t = g_t^k(X_t)$, such that
\begin{align}
  g_t^k(x) &= \int p_t(y) k(x,y) (\nabla \log p_*(y)-\nabla \log p_t(y)) dy\nonumber
  \\
  &=\int p_t(y) (k(x,y) \nabla \log p_*(y)+\nabla_y k(x,y)) dy 
\end{align}

Assume that $k(x,y) = \psi(x)^\top \psi(y)$, when the dimension of $\psi(x)\in \RR^D$ is finite, we have
\begin{align}
g_t^k(x) = \left(\int p_t(y) (\nabla \log p_*(y) \psi(y)^\top +\nabla \psi(y)^\top ) dy \right)\psi(x)
\end{align}

We can consider the function class as $s_\theta(x) = \theta \psi(x)$, $\theta\in\RR^{d\times D}$, then we can revisit kernelized gradient as an
analogue of score matching.

\begin{proposition}\label{prop:solution}
From the score matching view, when kernel feature map $\psi(x)\in\RR^D$, $s_\theta \in \{\theta\psi(x):\theta\in \RR^{d\times D}\}$, the score matching solution is
\begin{align}
\theta_t = \int p_t(y) \nabla \psi(y)^\top dy \left(\int p_t(y) \psi(y)\psi(y)^\top dy\right)^{-1}.
\end{align}

%score matching solution is NOT Stein kernel solution with a preconditioning matrix, 

%the score matching solution $\nabla\log p_t$
\end{proposition}

Proposition \ref{prop:solution} indicates that the $\nabla\log p_t$ on RKHS is generally not the optimal estimator for $\nabla \log p_t$, but with a (right) preconditioning matrix,
\begin{equation}\label{eq:precon}
  P_t^k =  \int p_t(y) \psi(y)\psi(y)^\top dy,
\end{equation}
which is the covariance matrix of feature map. Similarly, when $\nabla\log p_*(x) = \theta_*\psi(x)$, the kernelized gradient is 
$\theta_* \EE_{p_t(y)} \psi(y)\psi(y)^\top \psi(x)
$. Thus, we can conclude that the kernelized gradient is a (right) preconditioned gradient. There is a simple construction that when $\psi(x) = \Sigma_t^{-1/2}x$, such that $\Sigma_t = \EE_{p_t} xx^\top$, Eq. \eqref{eq:precon} becomes an identity matrix, which means that the kernelized gradient encounters true gradient. However, this construction entails the particle dependent kernel: $k(x,y)$ varies with different $p_t$. To better understand the effects of this preconditioning matrix, we consider the Gaussian transport task. 
%We focus on the repulsive term $\nabla \log p_t(x)$.
\begin{example}
 Consider that $\pi_t$ is $\mathcal N(\mu_t,\Sigma_t)$, $\pi_*$
 is $\mathcal N(\mu_*,\Sigma_*)$. The density function for $\mu_t$ and $\mu_*$ is $p_t$ and $p_*$. For Wasserstein gradient, $g_t^*(x) = \Sigma^{-1}_*(x-\mu_*)- \Sigma^{-1}_t(x-\mu_t)$. We consider two common kernel,
 
 (1) Linear kernel $k(x,y) = x^\top K y$, the corresponding $P_t^k = K^{\frac{1}{2}}\Sigma_t K^{\frac{1}{2}}$, 
 \begin{align}g^k_t(x) = \Sigma^{-1}_*
 K^{\frac{1}{2}}\Sigma_t
 K^{\frac{1}{2}} (x-\mu_*)-K(x-\mu_t)
 \end{align}
 
 (2) RBF kernel $k_\sigma(x,y) =\frac{1}{\sigma} \exp\left(-\frac{1}{2\sigma^2}\Vert x-y\Vert^2\right)$, 
 we have the update 
 \begin{align}
 g^{k_\sigma}_t(x) &= C_x \left(\left(\Sigma_*^{-1}-\Sigma_t^{-1}\right)\left( I + \sigma^{2}\Sigma_t^{-1}\right)^{-1}(x-\mu_t ) + 
    \Sigma_*^{-1} (\mu_t-\mu_*)\right)\\
    &= C_x\left(\Sigma_*^{-1} S_t(x-\mu_*) - \Sigma_t^{-1} S_t(x-\mu_t)
    + \Sigma_*^{-1}(I-S_t)(\mu_t-\mu_*)
    \right)
 \end{align}
 
 
    where $$C_x = \frac{1}{\sqrt{|\sigma^2 I +\Sigma_t|}}\exp\left(-\frac{1}{2\sigma^2}(x-\mu_t)^\top (I-S_t) (x-\mu_t)\right)$$
    $$
    0\prec S_t=(I+\sigma^2 \Sigma_t^{-1})^{-1}\prec I
    $$
 
    
 %the corresponding 
\end{example}

\iffalse
\begin{corollary}
For RBF kernel, 
$$
\lim_{\sigma\rightarrow0} S_t = I,\quad
\lim_{\sigma\rightarrow0} C_x = 0
$$
$$
\lim_{\sigma\rightarrow\infty} \sigma^2 S_t = \Sigma_t,\quad \lim_{\sigma\rightarrow\infty} \sigma^2 C_x = 1
$$
%\lim_{\sigma\rightarrow\infty}  S_t = 0,
\end{corollary}
\fi

Interestingly, 
with isotropic linear kernel, we found that the kernelized gradient accidentally provides better conditioning for the transportation, which makes particles converges easier than  plain Wasserstein gradient flow for ill-conditioned target distributions. 

For RBF kernel, although the preconditioning behavior is complex, the limiting cases of $\sigma$ lead to two outcomes: when $\sigma$ is large, $S_t\approx \Sigma_t/\sigma^2$, the preconditioning is similar to linear case; when $\sigma$ is small, $S_t\approx I$, the RBF kernelized gradient approaches Wasserstein gradient; but the scaling $C_x$ is ill-behaved in these two cases.

\iffalse
\begin{figure}[ht]
    \centering
    \begin{tabular}{ccc}
  \includegraphics[trim={1cm .5cm 1cm 1cm},clip,width=5cm]{figs/SM_path.pdf}  
        & \includegraphics[trim={1cm .5cm 1cm 1cm},clip,width=5cm]{figs/svgd_linear_path.pdf}
        & \includegraphics[trim={1cm .5cm 1cm 1cm},clip,width=5cm]{figs/opt_path.pdf}
\\
  \includegraphics[trim={1cm .5cm 1cm 1cm},clip,width=5cm]{figs/SM_T_5.00.pdf}  
        & \includegraphics[trim={1cm .5cm 1cm 1cm},clip,width=5cm]{figs/SVGD_T_5.00.pdf}
        & \includegraphics[trim={1cm .5cm 1cm 1cm},clip,width=5cm]{figs/opt_T_5.00.pdf}
\\
{\small (a) Without Preconditioning}&
{\small (b) SVGD $k(x,y)=x^\top y$}&
{\small (c) Optimal }\\
{\small $P_t = I$}&
{\small $P_t = \Sigma_t$}&
{\small $P_t = \Sigma_*$}
    \end{tabular}
    
   % \includegraphics[width=3.5cm]{figs/graph.png}
   
    \caption{Evolution of particle distribution from $\mathcal N([0,0]^\top,I)$ to $\mathcal N([20,20]^\top,\diag(100,1))$ (first row: evolution of particle mean $\mu_t$; second row: particle distribution $p_5(x)$ at $t=5$)
    }
    \label{fig:sde}
\end{figure}
\fi


\subsection{Two-sided Preconditioning}
%Beyond the kernel induced preconditioning, there are another type of 

As we mentioned in Section \ref{sec:comparison}, the main difference of SVGD and score matching is the preconditioning matrix. 
Such a preconditioning usually provides a better adaptation to the loss landscape geometry. 
Note that there are two types of preconditioning: left and right. For kernel design \citep{wang2019stein}, it produces a right-preconditioned gradient. Even the simplest isotropic linear kernel still produces a non-identical preconditioning.
The left-preconditioning is also widely used in practice, by implementing adaptive gradient optimizers,
such as Adam, RMSProp. 

%Previous work just take the usage of adaptive gradient for granted. Here, we have to highlight that it still plays an important role.

%A widely used technique in particle-based variational inference is preconditioning.  

%Previous works leverage preconditioning to boost the convergence of particles \citep{wang2019stein}.
%Also, Adam, and RMSProp are effective and popular optimizers in particle optimization setting. 



Considering the generalized version of Eq. \eqref{eq:transport},
\begin{equation}
    dX_t =  Q_t g_t(P_t X_t ) = Q_t (\nabla\log p_*(P_t X_t) - s_{\theta_t}(P_t X_t) ),
\end{equation}
where $Q_t$ and $P_t$ are time-dependent preconditioning matrix.

In real practice, the usage of preconditioning $P_t$ and $Q_t$ are similar. The algorithm can implement either $P_t$ or $Q_t$ in an efficient way. However, when the eigenvectors of $\Sigma_t$ and $\Sigma_*$ deviate significantly, $P_t$ and $Q_t$ behaves differently. 
We leave this phenomenon in the Appendix.


%However, we have to mention that the 

%Here, our framework also supports the precondition technique and

%Given a positive definite kernel $k(\cdot,\cdot): \RR^d\times\RR^d\rightarrow\RR$, and target distribution $\pi_*\propto\exp(-U(x))$ with well-defined $\nabla U$ on $\RR^d$.

\section{Theoretical properties of DSM}

TBA

\iffalse
\begin{assumption} (Smoothness and Convexity of $p_*$)
The distribution of $p_*$ is L-smoothness, \ie,
$$\int p_*(x)\Vert\nabla\log p_*(x)\Vert^2 dx <L .$$

Meanwhile, it satisfies $m$-log-Sobolev inequality
$$
J(p) = \int p(x)\left\Vert\nabla\log\frac{p(x)}{p_*(x)}\right\Vert^2 dx \geq 2m\mathcal L(p)
$$


\end{assumption}

\begin{assumption} (Smooth geodesic of $p_t$)
 For any $t>0$, $$\int p_t(x)\Vert\nabla\log p_t(x)\Vert^2 dx <L $$
\end{assumption}

\begin{assumption} ($\ep$-misspecification)
For any $t$,
 $$
 \min_\theta\int p_t(x) \Vert s_\theta(x) - \nabla \log p_t(x)\Vert^2 dx < \ep
 $$
\end{assumption}

\begin{assumption} ($\ep$-scaling)
We have
 $
  C_\ep =\ep/ m < 1
 $
\end{assumption}

\subsection{Continuous Case}


\begin{lemma}

$$
\frac{d\mathcal L(p_t)}{dt} = \int p_t(x) \left<\nabla \log p_*-s_\theta,\nabla \log p_*-\nabla \log p_t\right> dx
$$
\end{lemma}


\begin{corollary}

$$
\frac{d\mathcal L(p_t)}{dt} \leq -(1-C_\ep)m\mathcal L(p_t)
$$

$$
\mathcal L(p_t) \leq \mathcal L(p_0)\exp\left(-(1-C_\ep)mt\right)
$$
\end{corollary}

\fi
\subsection{Discrete Case}

\begin{algorithm}
\small
\DontPrintSemicolon
\KwInput{training data samples $\{z_i\}_{i=1}^n$, parametric model $p(z|x)=p_x(z):\mathcal Z\rightarrow \RR_+$, prior $p(x)$,
$s_\theta(x):\RR^d\rightarrow\RR^d$, 
Generator $G_\phi(x):\RR^d\rightarrow\RR^d$, 
initial parameters  $\theta_0,\phi_0$, noise sampler $X_0$,   
iteration parameter $T,T',T''$, learning rate $\eta,\eta'$, noise sample size $K$, particle sample size $m$
}
\For{$t=1,\dots,T$}{

Assign $\theta^0_t = \theta_{t-1} $;

\For{$t'=1,\cdots,T'$}{
\eIf{Randomized trace estimation}
 {Sample $\{\xi_i\}_{i=1}^K$, such that $\EE\xi=0$ and $\cov \xi = I$;
 
 Compute $\hat{L}(\theta) = \frac{1}{m}\sum_{i=1}^m \left(\Vert s_\theta(x_t^i)\Vert^2 + \frac{2}{K}\sum_{j=1}^K\xi_j^\top \nabla s_\theta(x) \xi_j\right) $
 }
 {Compute $\hat{L}(\theta) = \frac{1}{m}\sum_{i=1}^m \left(\Vert s_\theta(x_t^i)\Vert^2 + 2\nabla\cdot s_\theta(x_t^i)\right) $  }
 
 Update $\theta_t^{t'} = \theta_t^{t'-1} - \eta'\nabla \hat{L}(\theta_t^{t'-1})$;
}

Assign $\theta_t = \theta_{t}^{T'} $;

Compute unnormalized posterior log-density $\log p(x|z_1,\cdots,z_n)$: 
$
U(x) = - \sum_{i=1}^n\log p(x|z_i) - \log p(x)
$

Sample particles, $x^0_i = G_{\phi_{t-1}}(x_i)$, such that $x_i\sim X_0$ for all $i=1,\cdots,m$;

\For{$t''=1,\cdots,T''$}{
Update particles
$x_i^{t''}=x_i^{t''-1} - \eta  \left( \nabla U(x_i^{t''-1}) + s_{\theta_t}(x_i^{t''-1})\right)$ for all $i=1,\cdots,m$
}

Compute amotized loss $l(\phi) = \sum_{i=1}^m\Vert G_\phi(x_i)-x_i^{T''}\Vert^2$;

Update generator $\phi_t = \phi_{t-1}- \eta\nabla l(\phi_{t-1})$
%Update particles
%$x^i_t=x^i_t - \eta  \left( \nabla U(x_t^i) + s_{\theta_t}(x_t^i)\right)$ for all $i=1,\cdots,m$
}

\KwReturn{Generator $G_\phi$.}
\caption{Dynamical Score Matching (DSM): Amortized/Distilled Version}
\end{algorithm}


\section{Algorithm}

\subsection{Particle-based Algorithm}
Similar to SVGD, we first start with particle-based regime. We start with initial samples $x^0_1,\cdots,x^0_n\sim p_0(x)$, we would like to update these samples so that the distribution of final particles should be close to our target distribution $p_*(x)$.

\subsubsection{Parametric Repulsive Force}

For each time $t$, the estimation of $\nabla \log p_t(x)$ can be done by a function approximator, \ie, neural network parameterized by $\theta$, denoted as $s_\theta$.

\subsubsection{Parameter Reuse}





%Since that some 

\subsubsection{Randomized Trace Approximation}

Although $\nabla\cdot s_\theta(x)$ is tractable, the computation cost is about $d$ evaluations of $s_\theta$. When the distribution is high dimensional, the computation of $\nabla\cdot s_\theta$ increase significantly. To accelerate the computation of $\nabla s_\theta(x)$, we highlight that it is practical to use randomized trace approximation rather than exact computation.

\begin{proposition}
If $\EE\xi=0$ and $\cov \xi = I$, assume that $s^\xi_\theta(x) = s_\theta(x)^\top \xi$: $\RR^d\rightarrow\RR$ 
$$
\nabla\cdot s_\theta(x)=\EE\xi^\top \nabla s_\theta(x) \xi = \EE \xi^\top\nabla s^\xi_\theta(x).
$$
\end{proposition}



%\subsection{Amortized Algorithm}

%Similar to SVGD, the 

\section{Experiments}

\subsection{Density Sampling}

\subsubsection{Gaussian Mixture Distribution}
\begin{figure}[ht]
    \centering
    \begin{tabular}{ccc}
  \includegraphics[width=5cm]{figs/true1k.pdf}  
        & \includegraphics[width=5cm]{figs/svgd1k.pdf}
        & \includegraphics[width=5cm]{figs/our1k.pdf}
\\
{\small (a) True Density}&
{\small (b) Kernel Density}&
{\small (c)  Density (Ours)}
\\
  \includegraphics[width=5cm]{figs/true1k_sample.pdf}  
        & \includegraphics[width=5cm]{figs/svgd1k_sample.pdf}
        & \includegraphics[width=5cm]{figs/our1k_sample.pdf}
        \\
        {\small (d) True Samples}&
{\small (e) SVGD Samples}&
{\small (f)  Samples (Ours)}\\
  \includegraphics[width=5cm]{figs/true_score.pdf}  
        & \includegraphics[width=5cm]{figs/kernel_score.pdf}
        & \includegraphics[width=5cm]{figs/our_score.pdf}
        \\
        {\small (g) Stein Score}&
{\small (h) Kernelized Score}&
{\small (i) Estimated Score (Ours)}
    \end{tabular}
    
   % \includegraphics[width=3.5cm]{figs/graph.png}
   
    \caption{Particle-based density sampling for Gaussian mixture (10 clusters)
    }%parameterized by $\phi$
    %p_\theta(x,z,u) =
    %induced by $G_\theta^{-1}$
    \label{fig:dgm}
\end{figure}


%\subsubsection{Ill-conditioned Gaussian Distribution}

\subsection{Particle-based Bayesian Model}


\subsubsection{Bayesian Logistic Regression}

%\subsubsection{Bayesian Independent Component Analysis}

\begin{table}[H]
    \centering
\iffalse
    \begin{tabular}{c|c|cccc}
    \toprule
         &Sample size &   Accuracy & NLL & ECE &  Time\\
        \midrule
        \multirow{4}*{SVGD}&10&66.7&0.83&0.21&5.25
        \\
        &100
        & 69.0 &  0.61 &  0.17&5.71
        \\
        &1000&71.4 & 0.57 & 0.12&19.10\\
        &2000&76.2&0.55&0.11&81.50\\
        \midrule
        \multirow{4}*{DSM}&10
        &66.7& 0.84 & 0.21&7.95
        \\
        &100&
        71.4 & 0.56 & 0.12&8.15
        \\
        &1000&
        73.8 & 0.54 & 0.11&11.56
        \\
        &2000&
        76.2 & 0.54 & 0.11&13.22
        \\
        \bottomrule
    \end{tabular}
    \fi
        \begin{tabular}{c|c|cccc}
    \toprule
        Sample size &Algorithm &   Accuracy & NLL & ECE &  Time\\
        \midrule
        \multirow{2}*{10}&SVGD
        &66.7&\textbf{0.83}&0.21&\textbf{5.25}\\
        &DSM
        &66.7& 0.84 & 0.21&7.95
        \\
        \midrule
        \multirow{2}*{100}&SVGD
        &69.0 &  0.61 &  0.17&\textbf{5.71}\\
        &DSM
        &\textbf{71.4} & \textbf{0.56} & \textbf{0.12}&8.15
        \\
        \midrule
        \multirow{2}*{1000}&SVGD
        &71.4 & 0.57 & 0.12&19.10\\
        &DSM
        &\textbf{73.8} & \textbf{0.54} & \textbf{0.11}&\textbf{11.56}
        \\
        \midrule
        \multirow{2}*{2000}&SVGD
        &76.2&0.55&0.11&81.50\\
        &DSM
        &{76.2} & \textbf{0.54} & {0.11}&\textbf{13.22}
        \\
        \bottomrule
    \end{tabular}
    \caption{Bayesian logistic regression comparison (NLL: Negative Log-likelhood; ECE: Expected Calibration Error; Time: Time cost per 1,000 iteration)}
    \label{tab:my_label}
\end{table}

\subsubsection{Bayesian Neural Networks}


\subsection{Amortized Bayesian Model}

%    &=\int p_t(y) (\nabla \log p_*(y) k(x,y)+x) dy\\ &= \int p_t(y) \nabla \log p_*(y) y^\top K_t x dy+K_t x\\  &= (\EE_{p_t} \nabla \log p_*(y) y^\top K_t + K_t) x

%$\EE_{p_t} \nabla \log p_*(y) y^\top = -I
%$ if and only if $p_t = p_*$ (Stein's identity), The condition holds even if $\nabla \log p_*(y)$ is not linear.





%(1) If $p_*$ is NOT Gaussian, SM fails, SVGD is able to converge.

%(2) If $p_*$ is Gaussian, $K_t$ does not match $\Sigma_t^{-1}$, SVGD is not the steepest KL descent in Wasserstein space.

%Assume that $Y_t = K_t X_t$

%\begin{align*}
% &\text{SM: } &&dX_t = -(\Sigma_*^{-1}(X_t-\mu_*)-\Sigma_t^{-1}(X_t-\mu_t))  dt\\
% &\text{SVGD: } &&dX_t = -\left(\frac{1}{2}(\Sigma_*^{-1} \Sigma_t+\Sigma_t\Sigma_*^{-1} )K_t (X_t-\mu_*) - K_t (X_t-\mu_t) \right)  dt  
%\end{align*}




==> parts/body_v2_full.tex <==
\section{Analysis}




 \noindent\textbf{Notations.} In this paper, we use $x$ to denote particle samples in $\RR^d$. The distributions are assumed to be absolutely continuous w.r.t. the Lebesgue measure.
 The probability density function of the posterior is denoted by $p_*$.
 $p(t,x)$ (or $p_t$) refers to 
 particle distribution at time $t$.
 For scalar function $p(t,x)$, $\nabla_x p(t,x)$ denotes its gradient w.r.t. $x$. For vector function $g(t,x)$, $\nabla_x g(t,x)$, $\nabla_x\cdot g(t,x)$, $\nabla^2_x g(t,x)$ denote its Jacobian matrix, divergence, Hessian w.r.t. $x$. $\frac{\partial p(t,x)}{\partial t}$ and $\frac{\partial g(t,x)}{\partial t}$ denotes the partial derivative w.r.t. $t$.
 Without ambiguity, $\nabla$ stands for $\nabla_x$ for conciseness. Notation $\Vert x\Vert_H^2$ stands for 
 $x^\top H x$ and  $\Vert x\Vert_I$ is denoted by $\Vert x\Vert$. Notation $\Vert \cdot\Vert_{\cH^d}$  denotes the RKHS norm on $\RR^d$. 
 

%Notably,  it is well-known that Wasserstein gradient flow defines the first variation of $D_{\mathrm{KL}}(t)$ at $p(t,x)$ with a perturbation in Wasserstein space, such that $dX_t = \xi_t dt$, where $\xi_t$ is a random variable with bounded second moment. Then the KL Wasserstein gradient flow satisfies $\frac{\partial p(t,x)}{\partial t}= - \nabla \cdot [ p(t,x) \nabla\ln\frac{ p_*(x)}{p_t(x)} ].$ 

%When $\alpha=\infty$, there is not a stationary distribution, $X_t$ becomes a repulsive process with the heat equation.


%Using the definition above, the evolution of KL divergence satisfies
%\begin{align}\frac{d D_{\mathrm{KL}}}{d t}= -\int   p(t,x) [\nabla \cdot g(t,x) +  g(t,x) p(t,x)\nabla_x \ln {p_*(x)}] d x. \end{align}




%${d D_{\mathrm{KL}}}/{dt}$
We let $g(t,x)$ belong to a vector-valued function class $\cF$, and  find the best functional gradient direction. Inspired by the gradient boosting algorithm for regression and classification problems, we approximate the gradient flow by a function $g(t,x) \in \cF$ with a regularization term, which solves  the following minimization formulation:
\begin{equation}\label{eq:update}
    g(t,x) = \argmin_{f \in \cF} \left[-
\int   p(t,x) [\nabla \cdot f(x) +  f(x)^\top
\nabla \ln {p_*(x)} ] d x + Q({f})\right],
\end{equation}
where 
$Q(\cdot)$ is a regularization term that limit the output magnitude of $f$.
This regularization term also implicitly determines the underlying ``distance metric'' used to define the gradient estimates $g(t,x)$ in our framework. %As we show later, it can be regarded as a preconditioner to smooth the landscape of the Wasserstein gradient, similar to the role of Hessian matrix of Newton's method in the optimization literature. 
When $Q(x) = \frac{1}{2}\int p(t,x) \Vert f(x)\Vert^2 dx $,  Eq.~\eqref{eq:update} is equivalent to 
\begin{equation}\label{eq:wass2}
g(t,x)=\argmin_{ f\in\mathcal{{F}}}\int p(t,x) \left\Vert {f}(x)-\nabla \ln\frac{p_*(x)}{p_t(x)}\right\Vert^2 dx.
\end{equation}
If $\mathcal{F}$ is well-specified, i.e., $\nabla \ln\frac{p_*(x)}{p_t(x)}\in\cF$, we have $
g(t,x)=\nabla\ln\frac{p_*(x)}{p_t(x)},
$
which is the direction of Wasserstein gradient flow. Interestingly, despite the computational intractability of Wasserstein gradient, Eq.~\eqref{eq:update} provides a tractable variational approximation.
%$f_0$ is the base function such as $f_0(x)=0$, $f_0(x)=\nabla \log p_*(x)$, which provides a heuristic guidance for function learning.
%When $\ln p_t$ is differentiable, it is also possible to use the deterministic update $g(t,x)=\ln\frac{ p_*(x)}{p_t(x)}$ to mimic KL Wasserstein gradient flow.
 
% \noindent\textbf{Remark.}  Eq.~\eqref{eq:wass2} is obtained by using integration by parts. The converted version implies that the $\argmin$ operator is valid since $L_2$ norm is lower bounded by $0$.

 
 
 For RKHS, we will show that SVGD is a special case of Eq.~\eqref{eq:update}, where $Q(f) = \frac{1}{2}\Vert f\Vert_{\cH^d}^2$ (Sec. \ref{sec:svgd_reg}).  We point out that RKHS norm  cannot regularize the functional gradient properly since it is fixed for any $p(t,x)$.
 %due to the unconsciousness of $p(t,x)$.
 Our next example shows that SVGD is a suboptimal solution for Gaussian case.

%We have several examples to show that, SVGD with common kernels have issues even in Gaussian case.


% \noindent\textbf{Remark:}Thus, we choose Eq. \eqref{eq:reg} as our regularization.

%the regularization in RKHS cannot usually capture the Wasserstein gradient direction properly. 


%We leave the detailed derivation in Appendix \ref{appen:svgd}. 

%When $\cF$ is bounded, $Q(f)$ can be $0$, which encounters functional form of Frank-Wolfe algorithm as well as the Stein discrepancy. 

%Combining Eq. \eqref{eq:cont} and\eqref{eq:update}, the continuous version of proposed algorithm can be obtained.


%LIMITATION.
%(1) svgd as special; (2) limitation;

%We mainly focus on the properties of the dynamics with unbounded function class and regularization. In the following parts, we will show that with general function class beyond RKHS, the proposed algorithm is more practical and efficient than conventional SVGD. 

\iffalse
When the function class is bounded, we may apply functional form of Frank-Wolfe algorithm, which result in the Stein discrepancy,
\[
g(t,x) = \sup_{f \in \cF} 
\int   p(t,x) [\nabla \cdot f(x) +  f(x)^\top
\nabla \ln {p_*(x)}] d x .
\]
\fi


%\subsection{Gaussian case}

\begin{figure}[t]
    \centering
    \begin{tabular}{ccccc}
         \includegraphics[trim={0.8cm .7cm 1cm 1cm},clip,width=0.16\textwidth]{figs/svgd_linear_full.pdf}
        &\includegraphics[trim={0.8cm .7cm 1cm 1cm},clip,width=0.16\textwidth]{figs/rbf_full.pdf}
        &
          \includegraphics[trim={0.8cm .7cm 1cm 1.cm},clip,width=0.16\textwidth]{figs/true_star.pdf}  
        &\includegraphics[trim={0.8cm .7cm 1cm 1cm},clip,width=0.16\textwidth]{figs/pred_full.pdf}
        &
  \includegraphics[trim={0.8cm .7cm 1cm 1cm},clip,width=0.16\textwidth]{figs/opt_full.pdf}  
\\
{\tiny (a) $\frac{1}{2}\Vert f\Vert_{\cH^d}^2$ (linear)}&
{\tiny (b) $\frac{1}{2}\Vert f\Vert_{\cH^d}^2$ (RBF)}&
{\tiny (c) $\frac{1}{2}\EE_{p_t}\Vert f\Vert^2$ }&
{\tiny (d) $\frac{1}{2}\EE_{p_t}\Vert
f\Vert_{\Sigma_*^{-1}}^2
$ }&
{\tiny (e) Optimal transport}
\\
    \end{tabular}
    
   % \includegraphics[width=3.5cm]{figs/graph.png}
   
    \caption{Illustration of the functional gradient $g(t,x)$ compared with optimal transport. (a)-(d) denotes the corresponding $Q$ of the regularized functional gradient. (a)/(b) are SVGD with linear and RBF kernel. Optimal transport denotes the direction of the shortest path towards $p_*$.
    }
    \label{fig:exp_vec}
\end{figure}

\begin{figure}[t]
%\vspace{-0.3cm}
    \centering
    \begin{tabular}{cccc}
 \includegraphics[trim={0.8cm .7cm 1cm 1cm},clip,width=0.22\textwidth]{figs/svgd_linear_path_new.pdf}
        & \includegraphics[trim={0.8cm .7cm 1cm 1cm},clip,width=0.22\textwidth]{figs/svgd_rbf.pdf}
        &
      \includegraphics[trim={0.8cm .7cm 1cm 1cm},clip,width=0.22\textwidth]{figs/SM_path.pdf}  
        &
    \includegraphics[trim={0.8cm .7cm 1cm 1cm},clip,width=0.22\textwidth]{figs/opt_path.pdf}
\\
 \includegraphics[trim={0.8cm .7cm 1cm 1cm},clip,width=0.22\textwidth]{figs/svgd_linear_new.pdf}
        & \includegraphics[trim={0.8cm .7cm 1cm 1cm},clip,width=0.22\textwidth]{figs/svgd_rbf_t5.pdf}
        &
 \includegraphics[trim={0.8cm .7cm 1cm 1cm},clip,width=0.22\textwidth]{figs/SM_T_5_00.pdf}  
        &
        \includegraphics[trim={0.8cm .7cm 1cm 1cm},clip,width=0.22\textwidth]{figs/opt_T_5_00.pdf}
\\
{\tiny (a) $Q(f)=\frac{1}{2}\Vert f\Vert_{\cH^d}^2$ (linear)}&
{\tiny (b) $Q(f)=\frac{1}{2}\Vert f\Vert_{\cH^d}^2$ (RBF)}&
{\tiny (c) $Q(f)=\frac{1}{2}\EE_{p_t}\Vert f\Vert^2$ }&
{\tiny (d) $Q(f)=\frac{1}{2}\EE_{p_t}\Vert f\Vert_{\Sigma_*^{-1}}^2$ }
\end{tabular}
    
   % \includegraphics[width=3.5cm]{figs/graph.png}
   
    \caption{Evolution of particle distribution from $\mathcal N([0,0]^\top,I)$ to $\mathcal N([20,20]^\top,\diag(100,1))$ (first row: evolution of particle mean $\mu_t$; second row: particle distribution $p(5,x)$ at $t=5$)
    }
    \label{fig:sde}
%\vspace{-0.3cm}
\end{figure}


    %The first row indicate the 
    %attractive term: $\nabla\ln p_*(x)$ and its variational approximation;
   % The second row indicate the 
    %repulsive term $-\nabla\ln p_t(x)$ and its variational approximation. 


%Wasserstein gradient is the optimal choice.

\begin{example}\label{exp:breg}
 Consider that $p(t,\cdot)$ is $\mathcal N(\mu_t,\Sigma_t)$, $p_*$
 is $\mathcal N(\mu_*,\Sigma_*)$.  We consider the SVGD algorithm with linear kernel, RBF kernel, and regularized functional gradient formulation with $Q(f)=\frac{1}{2}\EE_{p_t}\Vert f\Vert^2$, and $Q(f)=\frac{1}{2}\EE_{p_t}\Vert f\Vert^2_{\Sigma_*^{-1}}$. Starting with $\mathcal N(0,I)$, 
 Fig.~\ref{fig:exp_vec} plots the $g(0,x)$ with different $Q$ and the optimal transport direction;
 the path of $\mu_t$ and $p(5,x)$ are illustrated in Fig.~\ref{fig:sde}. The detailed mathematical derivation are provided in the Appendix.
% (1) Linear kernel $k(x,y) = x^\top K y$,   \begin{align}g_{\mathrm{ker0}}(t,x) = - \Sigma^{-1}_*(\Sigma_* - \Sigma_t - (\mu_*-\mu_t)(\mu_*-\mu_t)^\top)x\end{align}
 %For optimal transport  $g_t^*(x) = -(x-\mu_*) + \Sigma_t^{-1/2} (\Sigma_t^{1/2}\Sigma_*\Sigma_t^{1/2})^{1/2}\Sigma_t^{-1/2}(x-\mu_t)$.

 %the corresponding 
\end{example}


Example \ref{exp:breg} shows the comparison of different regularizations for the functional gradient.
For RKHS norm, we consider the most commonly used kernels: linear and RBF. 
Fig. \ref{fig:exp_vec} shows the $g(0,x)$ of different regularizers: it is clear that only $Q(f)=\frac{1}{2}\EE_{p_t}\Vert f\Vert^2_{\Sigma_*^{-1}}$ approximates the optimal transport direction, while other $g(0,x)$ deviates significantly. 
SVGD with linear kernel underestimates the gradient of large-variance directions;
SVGD with RBF kernel even suffers from gradient vanishing in low-density area. 
Fig. \ref{fig:sde} demonstrates the path of $\mu_t$ with different regularizers.
For linear kernel, due to the curl component ($\mu_*\mu_t^\top$ term in linear SVGD is non-symmetric; See Appendix for details),  $p(5,x)$ is rotated with an angle.
For RBF kernel, it is misspecified (linear functions are not in $\cF$), leading to slow convergence. 
The $L_2$ regularizer is suboptimal due to the ill-conditioned $\Sigma_*$.
We can see that $Q(f)=\frac{1}{2}\EE_{p_t}\Vert f\Vert^2_{\Sigma_*^{-1}}$ produces the optimal path for $\mu_t$ (the line between $\mu_0$ and $\mu_*$). 

%Besides, the time-evolving term makes $K$ unable to perform preconditioning. Thus we let $K$ be $I$ in general.
%due to the $\mu_*\mu_t^\top$ term,
%For SVGD, as we indicated, linear kernel rotate the distribution and RBF kernel converges slow due to the gradient vanishing.

%under \noindent{[$\mathbf{A_3}$]}
\subsection{General Regularization}

%Proposition \ref{prop:equivalent} shows that for any $p_*$ and $p(t,x)$, the Mahalanobis regularization provides the preconditioned Wasserstein gradient.
%when $\cF$ contains the preconditioned Wasserstein gradient of KL divergence, i.e., $H^{-1}\nabla\ln \frac{p_*(x)}{p(t,x)}\in\cF$, and 
Inspired by the Gaussian case, we consider the general form
\begin{equation}\label{eq:reg}
 Q({f}(x))= \frac{1}{2}\int p(t,x) \Vert f(x)\Vert_H^2 dx 
\end{equation}
where $H$ is a symmetric positive definite matrix. 
Proposition \ref{prop:equivalent} shows that 
with Eq.~\eqref{eq:reg}, the resulting functional gradient is the approximation of preconditioned Wasserstein gradient flow. It also implies the well-definedness and existence of $g(t,x)$ when $\cF$ is closed, since $\Vert\cdot\Vert_H$ is lower bounded by 0. 

%it implies that the $ \EE_{p_t}f(x)^\top \nabla\ln p(t,x) $ term can be converted to $-\EE_{p_t} \nabla\cdot f(x)$.

%In particular, the $L_2$ regularization ($H=I$) leads to the approximation of Wasserstein gradient of KL divergence and $H$ implies different preconditioning design.

\begin{proposition}\label{prop:equivalent} Consider the case that $Q({f}) = \frac{1}{2}\int p(t,x) \Vert {f}(x)\Vert^2_H dx $, where $H$ is a symmetric positive definite matrix.  Then the functional gradient defined by Eq.~\eqref{eq:update} is equivalent as 
\begin{equation}\label{eq:def_g}
    g(t,x) =\argmin_{f\in\cF}
\frac{1}{2}\int   p(t,x) \left\Vert  {f}(x) - H^{-1} \nabla \ln \frac{p_*(x)}{p(t,x)}\right\Vert_H^2
 dx   
\end{equation}
\end{proposition}

%Our algorithm is an analogue of proximal gradient in Euclidean optimization.
\noindent\textbf{Remark.}  Our regularizer is similar to the
Bregman divergence in proximal gradient. 
We can further extend $Q(\cdot)$ with a convex function $h(\cdot):\RR\rightarrow [0,\infty)$, where the regularizer is defined by $Q({f}(x))= \EE_{p_t} h({f}(x))$. We can adapt more complex geometry in our framework with proper $h(\cdot)$.

%(1) It is possible to approximate Wasserstein gradient first and perform preconditioning. However, this needsthe computation of Hessian inverse, which is computationally intractable;(2) 

%and $\nabla \ln \frac{p_*(x)}{p(t,x)}\in\cF$.
%$\nabla \ln \frac{p_*(x)}{p(t,x)}$.

\subsection{Convergence analysis}\label{conv}

\paragraph{Equilibrium condition.}  To provide the theoretical guarantees, we show that the stationary distribution of our $g(t,x)$ update is $p_*$. Meanwhile, the evolution of KL-divergence is well-defined (without the explosion of functional gradient) and descending. We list the regularity conditions below.

\noindent{[$\mathbf{A_1}$]} (Regular function class)
The discrepancy induced by function class $\mathcal F$ is positive-definite: for any $q\neq p$, there exists $f\in\cF$ such that
$
\EE_q[\nabla \cdot f(x)+f(x)^\top \nabla \ln p(x)] >0
$. For $f\in\cF$ and $c\in\RR$, $cf\in\cF$, and $\cF$ is closed. The tail of $f$ is regular: $\lim_{\Vert x\Vert \rightarrow\infty} f(\theta,x) p_*(x) = 0$ for $f\in\mathcal{F}$.

\noindent{[$\mathbf{A_2}$]} ($L$-Smoothness) For any $x\in\RR^d$, $p_*(x)>0$ and $p(t,x)>0$ are $L$-smooth densities, \emph{i.e.}, $\Vert \nabla \ln p(x)-\nabla \ln p(y)\Vert\leq L\Vert x-y\Vert$, with $\EE_p\Vert x\Vert^2<\infty$.

Particularly, [$\mathbf{A_1}$] is similar to the positive definite kernel in RKHS, which guarantees the decrease of KL divergence. 
[$\mathbf{A_2}$] is designed to make the gradient well-defined: RHS of Eq.~\eqref{eq:evo} is finite.


%\noindent{[$\mathbf{A_3}$]} (Positive-definite)
%(Strongly convex regularization)
%The regularizer $Q$ and the corresponding $h$ satisfies
%$
%h(0) = 0,\quad h'(0)=0, \quad h(f)\geq\frac{\lambda}{2}f^2
%$, for some $\lambda>0$.

%\begin{assumption}\label{ass:regular} 
%\end{assumption}




\begin{proposition}\label{prop:equi}
Under $[\mathbf{A_1}]$, $[\mathbf{A_2}]$, when we update $X_t$ as Eq. (\ref{eq:def_g}), we have
$
-\infty <\frac{d D_{\mathrm{KL}}}{d t} < 0
$
 for all $p(t,x)\neq p_*(x)$.
\ie, 
$
g(t,x) = 0 \text{  if and only if $p(t,x)=p_*(x)$.}
$

\end{proposition}

 Proposition \ref{prop:equi} shows that the continuous dynamics of our $g(t,x)$ is well-defined and 
 the KL divergence along the dynamics is descending. The only stationary distribution for $p(t,x)$ is $p_*(x)$.
 %is well-behaved and descending. 

%provides convergence rate for \ModelName. 



\paragraph{Convergence rate.} The convergence rate of our framework mainly depends on (1) the capacity of function class $\cF$; (2) the complexity of $p_*$. In this section, we analyze that when the approximation error is small and the target $p_*$ is log-Sobolev, the KL divergence converges linearly. 



%\noindent{[$\mathbf{A_4}$]} Assume that $h$ is $L$-smooth,
%$
%\nabla^2 h(x) \preceq L I
%$.

\noindent{[$\mathbf{A_3}$]} ($\epsilon$-approximation) For any $t>0$, there exists $f_t(x)\in\cF$ and $\epsilon<1$, such that
{\footnotesize $$
\int p(t,x)\left\Vert
f_t(x) - 
H^{-1}\nabla\ln \frac{p(t,x)}{p_*(x)}\right\Vert_H^2 dx\leq \epsilon \int p(t,x)\left\Vert
\nabla\ln \frac{p(t,x)}{p_*(x)}\right\Vert_{H^{-1}}^2 dx
$$}




\noindent{[$\mathbf{A_4}$]}
 The target $p_*$ satisfies $\mu$-log-Sobolev inequality ($\mu>0$): For any differentiable function $g$, we have
 $
    \begin{aligned}
    \mathbb{E}_{p_*}\left[g^2\ln g^2\right]-\mathbb{E}_{p_*}\left[g^2\right]\ln \mathbb{E}_{p_*}\left[g^2\right]\le \frac{2}{\mu} \mathbb{E}_{p_*}\left[\left\|\nabla g\right\|^2\right].
    \end{aligned}
$


Specifically, [$\mathbf{A_3}$] is the error control of gradient approximation. With universal approximation theorem \citep{hornik1989multilayer}, any continuous function can be estimated by neural networks, which indicates the existence of such a function class. [$\mathbf{A_4}$] is a common assumption in sampling literature. It is more general than strongly concave assumption \citep{vempala2019rapid}. 
%For example, when $\ln p_*$ is strongly concave, it satisfies log-Sobolev inequality. 
%$$
%\int p(t,x)\ln \frac{p(t,x)}{p_*(x)} dx \leq \frac{1}{2\mu} \int p(t,x)\left\Vert\nabla\ln \frac{p(t,x)}{p_*(x)}\right\Vert^2 dx
%$$


\begin{theorem}\label{the:rate}
Under \noindent{$[\mathbf{A_1}]$}-\noindent{$[\mathbf{A_4}]$}, for any $t>0$, we assume that the largest eigenvalue, $\lambda_{\max}(H)=m$. Then we have $\frac{d D_{\mathrm{KL}}(t)}{dt}\leq -\frac{1-\epsilon}{2}\mathbb{E}_{p_t} \left\|\nabla \ln \frac{p_t(x)}{p_*(x)}\right\|^2_{H^{-1}}
$ and
$
D_{\mathrm{KL}}(t) \leq \exp(-(1-\epsilon)\mu t/m) D_{\mathrm{KL}}(0).
$

\end{theorem} 

Theorem \ref{the:rate} shows that when $p_*$ is log-Sobolev, our algorithm achieves linear convergence rate 
with a function class powerful enough to approximate the preconditioned Wasserstein gradient. Moreover, considering the discrete algorithm, we have to make sure that the step size is proper, \emph{i.e.}, $\Vert H^{-1}\nabla^2\ln p_*(x)\Vert \leq c $, for some constant $c>0$. Thus, the preconditioned $H = -c\nabla^2 \ln p_*$ is better than plain one $H = cLI$, since $(-\nabla^2 \ln p_*)^{-1}\succeq L^{-1}I$. For better understanding, we have provided a Gaussian case discretized proof in Appendix 
\ref{sec:gauss_dis} to illustrate this phenomenon. 

%In real practice, to obtain a proper learning rate, $\Vert H^{-1}\nabla^2\ln p_*\Vert_2\leq 1$ is used in optimization 

%for discretized algorithm









\section{PFG: Preconditioned Functional Gradient Flow}

\begin{algorithm}
\small
\DontPrintSemicolon
\KwInput{ Unnormalized target distribution $p_*(x) =e^{-U(x)}$, 
$f_\theta(x):\RR^d\rightarrow\RR^d$, 
%$f_0(x):\RR^d\rightarrow\RR^d$,
 initial particles (parameters) $\{x^i_0\}_{i=1}^n$, $\theta_0$, 
iteration parameter $T,T'$, step size $\eta,\eta'$, regularization function $h(\cdot)$.
}
\For{$t=1,\dots,T$}{

Assign $\theta^0_t = \theta_{t-1} $;

\For{$t'=1,\cdots,T'$}{
 {Compute $\hat{L}(\theta) = \frac{1}{n}\sum_{i=1}^n \left( h(f_\theta(x_t^i)) + f_\theta(x_t^i)\cdot \nabla U(x_t^i) - \nabla\cdot f_\theta(x_t^i)\right) $  }
 
 Update $\theta_t^{t'} = \theta_t^{t'-1} - \eta'\nabla \hat{L}(\theta_t^{t'-1})$;
}

Assign $\theta_t = \theta_{t}^{T_1} $ and update particles
$x^i_t=x^i_t + \eta  \left(  f_{\theta_t}(x_t^i)\right)$ for all $i=1,\cdots,n$;
}

\KwReturn{Optimized particles $\{x^i_T\}_{i=1}^n$}
\caption{PFG: Preconditioned Functional Gradient Flow}
\label{alg}
\end{algorithm}

%\vspace{-0.2cm}
\subsection{Algorithm}

We will realize our algorithm with parametric $f_\theta$ (such as neural networks) and discretize the update.

\noindent\textbf{Parametric Function Class.} We can let 
$
\cF=\{f_\theta(x):\theta\in\Theta  \}$
and apply $g(t,x) = {f}_{\hat{\theta}_t}(x) $, such that
\begin{equation}\label{eq:general}
  \hat{\theta}_t=\argmin_{\theta\in\Theta} \left[
\int   p(t,x) [-\nabla \cdot f_\theta(x) - f_\theta(x)^\top
\nabla \ln {p_*(x)} + \frac{1}{2}\Vert{f}_\theta(x)\Vert_{H}^2 ] d x 
 \right],  
\end{equation}

where $H$ is a symmetric positive definite matrix estimated at time $t$.   Eq.~\eqref{eq:general} is a direct result from Eq.~\eqref{eq:update} and \eqref{eq:reg}. The  parametric function class allows ${f}_\theta$ to be optimized by iterative algorithms. %Besides, by Proposition \ref{prop:equivalent}, our $f_\theta$ is approximate the $\nabla\ln \frac{p_*}{p_t}$.

%Thus, the $L_2$ regularization in our formulation leads to the approximation of Wasserstein gradient of KL divergence.
%\begin{proposition} 
%The functional gradient 
%$f_H$ induced by \eqref{eq:hermitian} is equivalent with $H f_I$, where $H$ is a preconditioning matrix for functional gradient $f_I$ induced by $L_2$ regularization. 
%\end{proposition}
%We will provide an example below to illustrate the geometric interpretation for the Bregman regularization and make some comparison with the kernel geometry.
%According to our analysis, the optimal $H$ should be $-\nabla^2\ln p_*$.
%to either function output or parameter scaling directly.
%We highlight that the regularization in this form has meaningful interpretation in Wasserstein gradient flow. We will discuss in the following parts.
\noindent\textbf{Choice of $H$.} Considering the posterior mean trajectory, it is equivalent to the conventional optimization, so that $-\nabla^2\ln p_*$ is ideal (Newton's method) to implement discrete algorithms.
We use diagonal Fisher information estimators for efficient computation as Adagrad
\citep{duchi2011adaptive}. We approximate the preconditioner $H$ for all particles at each time step $t$ by moving averaging.

%In our experiments, we use diagonal estimation for simplicity.includes Kronecker-factored (KFAC)  \citep{martens2018kronecker}
%, which can be estimated by Fisher information  \citep{methodology1989likelihood}
%For large experiments, we use diagonal estimation.
% which can be obtained by Kronecker-factored (KFAC) approximation \citep{martens2018kronecker}
\noindent\textbf{Discrete update.} We can present our algorithm by discretizing Eq.~\eqref{eq:update} and \eqref{eq:general}. Given $X_0\sim p_0$, we update $X_k$ as $
X_{k+1} = X_k + \eta {f}_{\hat{\theta}_k}(X_k),
$
where 
$  \hat{\theta}_k
$ is obtained by Eq.~\eqref{eq:general} with (stochastic) gradient descent. The integral over $p(k,x)$ is estimated by particle samples.   Full procedure is presented in Alg. \ref{alg}, where the regularizer $h$ is $\frac{1}{2}\Vert\cdot\Vert_H^2$ by default.



\subsection{Comparison with SVGD}
\subsubsection{SVGD from Functional Gradient View}\label{sec:svgd_reg}

For simplicity, we prove the case under finite-dimensional feature map\footnote{Infinite-dimensional version is provided in Appendix \ref{sec:inf}.}, $\psi(x):\RR^d\rightarrow\RR^h$.
We assume that 
$
\cF= \{ W \psi(x): W\in\RR^{d\times h}\} ,
$
and let kernel
$
k(x,y) = \psi(x)^\top \psi(y) ,
$  $Q(f)=\frac{1}{2}\Vert f\Vert_{\cH^d}^2=\frac{1}{2}\Vert W\Vert_F^2$, where RKHS norm is the Frobenius norm of $W$.
The solution is defined by
\begin{equation}
    \hat{W}_t = 
\argmin_{W\in\RR^{d\times h}} 
-\int   p(t,x) \trace[W \nabla \psi(x) +  W \psi(x)
\nabla \ln {p_*(x)}^\top] d x + \frac{1}{2}\Vert W\Vert_F^2,
\end{equation}
which gives
$
\hat{W}_t = 
\int   p(t,x') [\nabla \psi(x')^\top +
 \nabla \ln {p_*(x')} \psi(x')^\top] d x' .
$
This implies that 
\begin{equation}
g(t,x)=\hat{W}_t \psi(x)
= \int   p(t,y) [\nabla_{y} k(y,x)+
\nabla \ln {p_*(y)} k(y,x)] d y,
\end{equation}
which is equivalent to SVGD. For linear function classes, such as RKHS, $Q$ can be directly applied to the parameters, such as $W$ here. The regularization of
SVGD is $\frac{1}{2}\Vert \cdot\Vert^2_F$ (the norm defined in RKHS).  
For non-linear function classes, such as neural networks, the RKHS norm cannot be defined.



 %When $H=I$, $\alpha=\infty$, it becomes the score matching loss.

\subsubsection{Limitations of SVGD}\label{sec:limit}

\noindent \textbf{Kernel function class.} As in Section \ref{sec:svgd_reg}, RKHS only contains linear combination of the feature map functions, which suffers from curse of dimensionality \citep{geenens2011curse}. On the other hand, some non-linear function classes, such as neural network,  performs well on high dimensional data \citep{lecun2015deep}. The extension to non-linear function classes is needed for better performance.

%with predefined feature map $\psi(x)$
%Thus, 
%From the theoretical view, even with log-Sobolev target distribution, SVGD with common kernels fails to achieve the linear rate, while Wasserstein gradient flow can obtain. The extension to larger function class is needed.
%the function class of our framework extend the RKHS to unbounded function classes. 
%From the theoretical view, our function class provides linear convergence rate for log-Sobolev target distribution, while SVGD with common kernels fails to achieve the rate.
%When target distribution is shifted with a constant vector, we would like to find an algorithm to correct the shifted vector quickly. Unfortunately, the SVGD algorithm fails to obtain the optimal geodesic in general and the kernel design cannot fix it.
\noindent \textbf{Gradient preconditioning in SVGD.} In Example \ref{exp:breg}, when $-\nabla^2 \ln p_*$ is ill-conditioned, PFG algorithm follows the shortest path from $\mu_0$ to $\mu_*$. 
Although SVGD can implement preconditioning matrices as \citep{wang2019stein}, due to the curl component and time-dependent Jacobian of $d\mu_t/dt$, any symmetric matrix cannot provide optimal preconditioning (detailed derivation in Appendix).

%Although $K$ in SVGD with linear kernel can be designed, due to the coupling with $\mu_*\mu_t^\top$ in $g(t,x)$, any symmetric $K$ cannot provide proper preconditioning for SVGD algorithm (detailed derivation in Appendix).
%Although SVGD is a moment matching algorithm, due to the global constraint of RKHS, the  of the SVGD algorithm is usually hard to control.
%As shown in Example \ref{exp:breg}, SVGD differs from Wasserstein gradient significantly. It also suffers from the ill-conditioning. Figure \ref{fig:exp_vec} provides visualization for the Wasserstein gradient, SVGD, and optimal transport, and our algorithm. With proper regularization, our algorithm approximate the optimal transport direction. Nonetheless, Wasserstein gradient and SVGD deviate significantly.
%\begin{proposition}\label{prop:mean} (Mean matching) Assume that $p_t(x) = p_*(x+b)$, where $b$ is a constant vector shift. The optimal transport from $p_t$ to $p_*$ satisfies $g(t,x) \propto b$.\end{proposition}
%Proposition \ref{prop:mean} shows that the underlying variational gradient needs to detect the shift direction to obtain the optimal . However, when $\nabla\ln\frac{p_*}{p_t}$ is ill-conditioned, both Wasserstein gradient and SVGD cannot obtain a proper direction towards target mean. Our next example shows the impacts of different regularizations.
%Section \ref{sec:svgd_reg} indicate that the behavior of direct regularization over parameters in non-linear function space is not clear. 
%We found that even in linear function space, the kernel design is still challenging with the Hilbert regularization. 
%We provide an example to show that even in Gaussian case,  SVGD with common kernels suffers from different issues.
%The introduction of Bregman regularization brings preconditioning matrix to our algorithm. Due to the function class design, our Bregman regularization is more flexible than kernel design in RKHS. As in Example \ref{exp:breg}, the preconditioning matrix of our framework is independent of $\Sigma_t$, while SVGD has to deal with this term. This property makes SVGD unable to provide Hessian-inverse preconditioning with a time-independent kernel.
%For SVGD, the kernel design $k(x,y)$ is provided. The optimal one denotes the optimal transport of from $p_t$ to $p_*$, which differs from the Wasserstein gradient.
%Example \ref{exp:breg} shows that due to the fixed design of function bias term $c$ in Eq.~\eqref{eq:linear_ker}, preconditioning matrix is 
%the SVGD cannot approximate both attractive and repulsive term well with one linear kernel.
%When bias term is $\mu_*$, the resulting estimation of $\nabla \ln p(t,x)$ is heavily biased. 
%When bias term is $\mu_t$, the resulting estimation of $\nabla \ln p_*(x)$ fails and the expectation of $p_t$ stucks at $\mu_t$.
%In particular, when we regularize the function output directly with samples from $p(t,x)$, and the function class is well-specified (linear function class for Gaussian), 
%Wasserstein gradient. For example, in case (1), Thus, we have to choose different bias term for $\nabla \ln p_*(x)$ and $\nabla \ln p(t,x)$ separately, which is not practical. Considering the comparison between (2) and (3), we can see that the precondition term of $\ln p_*(x)$ in RKHS produces a $\Sigma_t^{-1}$, that means the preconditioning of it becomes hard due to the time dependency.
%But our extension to larger function class makes it possible.
\noindent \textbf{Suboptimal convergence rate.} 
For log-Sobolev $p_*$, 
SVGD with commonly used bounded smoothing kernels (such as RBF kernel) cannot reach the linear convergence rate \citep{duncan2019geometry} and the explicit KL convergence rate is unknown yet.
Meanwhile, the Wasserstein gradient flow converges linearly. When the function class is sufficiently large, PFG converges provably faster than SVGD. 
%Our  approximate the Wasserstein gradient 

\noindent \textbf{Computational cost.} For SVGD, main computation cost comes from the kernel matrix: with $n$ particles, we need $O(n^2)$ memory and computation. Our algorithm uses an iterative approximation to optimize $g(t,x)$, whose memory cost is independent of $n$ and computational cost is $O(n)$ \citep{bertsekas2011incremental}. 
The repulsive force between particles is achieved by $\nabla\cdot f$ operator on each particle.

%For solutions with $\epsilon$ error tolerance, iterative approximation algorithm () converges in $O(n/\epsilon^2)$.


%As we mentioned, the 
\section{Experiment}\label{exp}

To validate the effectiveness of our algorithm, we have conducted experiments on both synthetic and real datasets. Without special declarations, we use parametric two-layer neural networks with Sigmoid activation as our function class. To approximate $H$ in real datasets, we use the approximated diagonal Hessian matrix $\hat H$, and choose $H = \hat H^\alpha$, where $\alpha\in \{0,0.1,0.2,0.5,1\}$;
the inner loop $T'$ of PFG is chosen from $\{1,2,5,10\}$, the hidden layer size is chosen from $\{32,64,128,256,512\}$. The parameters are chosen by validation.
 More detailed settings are provided in the Appendix.
 
 %For functional gradient initialization, we conduct a warm-start stage at the beginning, where samples are sampled from $p(0,x)$ to obtain $g(0,x)$.
%The optimizer is Adam without momentum.

%\subsection{Synthetic Experiments}\label{sec:density}



%In this part, our method use linear function class and regularization $Q(f) = \EE_{p_t}\Vert f(x)\Vert_{\Sigma_*^{-1}}$.
%The Wasserstein gradient is a special case of our algorithm to obtain the tractable form.
%when $\mu_*$ is small and $\Sigma_*$ is ill-conditioned, the 




\begin{figure}[t]
    \centering
    \begin{tabular}{ccc}
  \includegraphics[trim={0.2cm .2cm .2cm .2cm},clip,width=0.3\textwidth]{figs/true10k.pdf}  
        & \includegraphics[trim={0.2cm .2cm .2cm .2cm},clip,width=0.3\textwidth]{figs/svgd1k.pdf}
        & \includegraphics[trim={0.2cm .2cm .2cm .2cm},clip,width=0.3\textwidth]{figs/dsm_new.pdf}
\\
{ (a) True Density}&
{ (b) SVGD Density }&
{ (c) PFG Density }
\\
  \includegraphics[trim={0.2cm .2cm .2cm .2cm},clip,width=0.3\textwidth]{figs/true1k_sample.pdf}  
        & \includegraphics[trim={0.2cm .2cm .2cm .2cm},clip,width=0.3\textwidth]{figs/svgd1k_sample.pdf}
        & \includegraphics[trim={0.2cm .2cm .2cm .2cm},clip,width=0.3\textwidth]{figs/our1k_sample.pdf}
        \\
        { (d) True Samples}&
{ (e) SVGD Samples}&
{ (f) PFG Samples }\\
  \includegraphics[trim={0.2cm .2cm .2cm .2cm},clip,width=0.3\textwidth]{figs/true_score.pdf}  
        & \includegraphics[trim={0.2cm .2cm .2cm .2cm},clip,width=0.3\textwidth]{figs/kernel_score.pdf}
        & \includegraphics[trim={0.2cm .2cm .2cm .2cm},clip,width=0.3\textwidth]{figs/our_score.pdf}
        \\
        { (g) Stein Score}&
{ (h) SVGD Score}&
{ (i) PFG Score }
    \end{tabular}
    \caption{Particle-based VI for Gaussian mixture sampling.
    }%parameterized by $\phi$
    %p_\theta(x,z,u) =
    %induced by $G_\theta^{-1}$
    \label{fig:dgm}
    \vspace{-0.2cm}
\end{figure}

\noindent\textbf{Gaussian Mixture.} To demonstrate the capacity of non-linear function class,  we have conducted the Gaussian mixture experiments to show the advantage over linear function class, e.g., SVGD (RBF kernel). We consider to sample from a 10-cluster Gaussian Mixture distribution. Both SVGD and our algorithm are trained with 1,000 particles. 
Fig. \ref{fig:dgm} shows that  the estimated score by RBF kernel is usually unsatisfactory: (1) In low-density area, it suffers from gradient vanishing, which makes samples stuck at these parts (similar to Fig.~\ref{fig:exp_vec} (b)); (2) The score function cannot distinguish connected clusters.
Specifically, some clusters are isolated while others might be connected. The choice of bandwidth is hard. The fixed bandwidth makes the SVGD algorithm unable to determine the gradient near connected clusters. It fails to capture the clusters near $(-0.75,0.5)$. However, the non-linear function class is able to resolve the above difficulties. In PFG, we found that the score function is well-estimated and the resulting samples mimic the true density properly.


\begin{figure}[t]
%\vspace{-0.3cm}
    \centering
    \begin{tabular}{cccc}
       \multicolumn{4}{c}{\includegraphics[trim={7.cm 0.5cm 7cm 0.5cm},clip,width=0.8\textwidth]{figs/legend.pdf} }\\
  \includegraphics[trim={0.cm .0cm 0cm 0cm},clip,width=0.22\textwidth]{figs/mu_sigma1_1.pdf}  
        & \includegraphics[trim={0.cm .0cm 0cm 0cm},clip,width=0.22\textwidth]{figs/mu_1.pdf}
        & \includegraphics[trim={0.cm .0cm 0cm 0cm},clip,width=0.22\textwidth]{figs/mu_sigma1.pdf}
        & \includegraphics[trim={0.cm .0cm 0cm 0cm},clip,width=0.22\textwidth]{figs/mu_20.pdf}
\\
  \includegraphics[trim={0.cm 0.cm 0cm 0cm},clip,width=0.22\textwidth]{figs/kl_sigma1_1.pdf}  
        & \includegraphics[trim={0.cm .0cm 0cm 0cm},clip,width=0.22\textwidth]{figs/kl_1.pdf}
        & \includegraphics[trim={0.cm .0cm 0cm 0cm},clip,width=0.22\textwidth]{figs/kl_sigma1.pdf}
        & \includegraphics[trim={0.cm .0cm 0cm 0cm},clip,width=0.22\textwidth]{figs/kl_20.pdf}
        \\
    {\tiny (a) $\mu_*=[1,1]^\top$}&
{\tiny(b) $\mu_*=[1,1]^\top$}&
{\tiny(c) $\mu_*=[20,20]^\top$}&
{\tiny(d) $\mu_*=[20,20]^\top$ }\\
{\tiny $\Sigma_*=\diag(1,1)$}&
{\tiny $\Sigma_*=\diag(100,1)$}&
{\tiny  $\Sigma_*=\diag(1,1)$}&
{\tiny  $\Sigma_*=\diag(100,1)$ }
     
\end{tabular}
    
   % \includegraphics[width=3.5cm]{figs/graph.png}
   
    \caption{Evolution of particle distribution from $\mathcal N(0,I)$ to $\mathcal N(\mu_*,\Sigma_*)$ (first row: mean squared error of $\mu_t$: $\Vert \mu_t-\mu_*\Vert^2$; second row: KL divergence between $p(t,x)$ and $p_*(x)$)
    }
    \label{fig:kl}
  
\end{figure}
\noindent\textbf{Ill-conditioned Gaussian distribution.} We show the effectiveness of our proposed regularizer. For ill-conditioned Gaussian distribution, the condition number of $\Sigma_*$ is large, \ie, the ratio between maximal and minimal eigenvalue is large.
We follow Example \ref{exp:breg} and compare different $\mu_*$ and $\Sigma_*$.
When $\Sigma_*$ is well-conditioned ($\Sigma_* = I$), $L_2$ regularizer (equivalent to Wasserstein gradient) performs well.
However, it will be slowed down significantly with ill-conditioned $\Sigma_*$. 
For SVGD with linear kernel, the convergence slows down with shifted $\mu_*$ or ill-conditioned $\Sigma_*$. For SVGD with RBF kernel, the convergence is slow due to the misspecified function class. Interestingly, for ill-conditioned case, $\mu_t$ of SVGD (linear) converges faster than our method with $H=I$ but KL divergence does not always follow the trend. The reason is that $\Sigma_t$ of SVGD is highly biased, making KL divergence large. Our algorithm provides feasible Wasserstein gradient estimators and makes the particle-based sampling algorithm compatible with ill-conditioned sampling case.


%\subsection{Approximate Posterior Inference}




\noindent \textbf{Logistic Regression.} We conduct Bayesian logistic regression for binary classification task on Sonar and Australian dataset \citep{uci}. In particular, the prior of weight samples are assigned $\mathcal{N}(0,1)$; the step-size is fixed as $0.01$.
We compared our algorithm with SVGD (200 particles), full batch gradient is used in this part. 
To measure the quality of posterior approximation, we use 3 metrics: (1) the distance between sample mean $\mu_t$ and posterior mean $\mu_*$; (2) the Maximum Mean Discrepancy (MMD) distance \citep{gretton2012kernel} from particle samples to posterior samples; (3) the evidence lower bound (ELBO) of current particles,
${\EE}_{x\sim p_t}\left[\log {p}_*(x)-\log p(t,x)\right]$,  where
${p}_*(x)$ is the unnormalized density $p(x,\cD)$ with training data $\cD$,
the entropy term $\log p(t,x)$ is estimated by kernel density.
The ground truth samples of $p_*$ is estimated by NUTS \citep{hoffman2014no}. Fig. \ref{fig:logistic} shows that our method outperforms SVGD consistently.
\begin{figure}[H]
   
    \centering
    \includegraphics[trim={14.cm 0.5cm 14cm 0.5cm},clip,width=0.5\textwidth]{figs/legend4.pdf}
    \begin{tabular}{ccc}
  \includegraphics[width=0.3\textwidth]{figs/mse_.pdf}  
        &  \includegraphics[width=0.3\textwidth]{figs/mmd_.pdf}
        &  \includegraphics[width=0.3\textwidth]{figs/elbo_.pdf}\\
        \includegraphics[width=0.3\textwidth]{figs/mse_a_.pdf}  
        & \includegraphics[width=0.3\textwidth]{figs/mmd_a_.pdf}
         & \includegraphics[width=0.3\textwidth]{figs/elbo_a_.pdf}
    \end{tabular}
    
   % \includegraphics[width=3.5cm]{figs/graph.png}
   %Numbers in x-axis stands for $n$ thousands iterations.
    \caption{ Posterior sampling for Bayesian logistic regression. (200 particles; dataset: \emph{sonar} (first row) and \emph{Australian} (second row). $\mu_t$: particle mean; $\mu_*$: posterior mean.)
    }
   % \vspace{-0.5cm}%parameterized by $\phi$
    %p_\theta(x,z,u) =
    %induced by $G_\theta^{-1}$
    \label{fig:logistic}
\end{figure}



\noindent \textbf{Hierarchical Logistic Regression.} For hierarchical logistic regression, we consider a 2-level hierarchical regression, where prior of weight samples is $\mathcal{N}(0,\alpha^{-1})$. The prior of $\alpha$ is $\text{Gamma}(0,0.01)$.
All step-sizes are chosen from $\{10^{-t}:t=1,2,\cdots\}$ by validation.
We compare the test accuracy and negative log-likelihood as \citet{liu2016stein}. Mini-batch was used to estimate the log-likelihood of training samples (batch size is 200).
Tab. \ref{tab:hir} shows that our algorithm performs the best against SVGD and SGLD on hierarchical logistic regression.

\begin{table}[H]
    \centering
 %   \vspace{-0.4cm}
   
  \caption{Hierarchical Logistic Regression on UCI datasets (particle size = 200)}
     % &{}&\multicolumn{3}{c}{German}\\
%    \midrule
\vspace{0.2cm}
  \begin{sc}
  \begin{tabular}{c|cccc}
  \toprule
     & \multicolumn{2}{c}{covtype} & \multicolumn{2}{c}{german} \\
     & acc.          & nll         & acc.         & nll         \\
     \midrule
SVGD &     75.1          &     0.58        &    65.1          &        0.71     \\
SGLD &      74.9         &    0.57         &    64.8          &     0.65     \\
PFG &         \textbf{75.7}  &       \textbf{0.51}      &    \textbf{67.6}         &     \textbf{0.64}   \\
\bottomrule
\end{tabular}
    \end{sc}
    \label{tab:hir}
  %  \vspace{-0.2cm}
\end{table}



\noindent \textbf{Bayesian Neural Networks.} We compare our algorithm with SGLD and SVGD variants
on Bayesian neural networks. We conduct the two-layer network with 50 hidden units (100 for Year dataset, 128 for MNIST) and ReLU activation function; the batch-size is 100 (1000 for Year dataset), All step-sizes are chosen from $\{10^{-t}:t=1,2,\cdots\}$ by validation.
For UCI datasets,  we choose the preconditioned version for comparison: M-SVGD \citep{wang2019stein} and pSGLD
\citep{li2016preconditioned}.
Data samples are randomly partitioned to two parts: 90\% (training), 10\% (testing) and 
 100 particles is used.
 For MNIST, 
 data split follows the default setting and we compare our algorithm with SVGD 
 for $5,10,50,100$ particles (SVGD with 100 particles exceeded the memory limit). In Tab. \ref{tab:uci_bnn}, PFG outperforms SVGD and SGLD significantly.
 In Fig.~\ref{fig:BNN}, we found that the accuracy and NLL of PFG is better than SVGD with all particle size. With more particle samples, PFG algorithm also improves. 
 
%For UCI dataset,

 
\begin{table}[H]
   
    \caption{
    Averaged test root-mean-square error
 (RMSE) and test log-likelihood of Bayesian Neural Networks on UCI datasets (100 particles). Results are computed by 10 trials.}\label{tab:uci_bnn}
 \vspace{0.15in}
 \centering
\begin{sc}
    \begin{tabular}{c|ccc|ccc}
\toprule  & \multicolumn{3}{c|}{ { Average Test RMSE }}&\multicolumn{3}{c}{ { Average Test Log-likelihood }} \\
{ Dataset } &  { M-SVGD } & { pSGLD } & { \ModelName }& { M-SVGD } & { pSGLD } & { \ModelName } \\
\midrule { Boston } 
& 2.72$_{\pm0.17}$ 
& 2.70$_{\pm0.16}$ 
& \textbf{2.47}$_{\pm0.11}$
&-2.86$_{\pm0.20}$
&-2.85$_{\pm0.18}$
&\textbf{-2.35}$_{\pm0.12}$
\\
{ Concrete } & 4.83$_{\pm0.11}$
&5.05$_{\pm0.13}$&
\textbf{4.69}$_{\pm0.14}$
&-3.21$_{\pm0.06}$&
-3.21$_{\pm0.07}$&
\textbf{-2.83}$_{\pm0.16}$
\\
{ Energy } & 0.89$_{\pm0.10}$ 
&0.99$_{\pm0.08}$ &
\textbf{0.48}$_{\pm0.04}$
&-1.42$_{\pm0.03}$
&-1.31$_{\pm0.05}$
&\textbf{-1.22}$_{\pm0.06}$
\\
{ Protein } & 4.55$_{\pm0.14}$
&4.59$_{\pm0.18}$&
\textbf{4.51}$_{\pm0.06}$
&-3.07$_{\pm0.13}$
&-3.22$_{\pm0.11}$
&\textbf{-2.89}$_{\pm0.07}$
\\
{ WineRed } & 0.63$_{\pm0.04}$ 
&0.64$_{\pm0.02}$ &
\textbf{0.60}$_{\pm0.02}$
&-1.77$_{\pm0.05}$&
-1.80$_{\pm0.08}$&
\textbf{-1.61}$_{\pm0.03}$
\\
{ WineWhite } & 0.65$_{\pm0.05}$ 
&0.67$_{\pm0.07}$ &
\textbf{0.59}$_{\pm0.02}$
&-1.75$_{\pm0.04}$
&-1.82$_{\pm0.07}$
&\textbf{-1.58}$_{\pm0.04}$
\\
{ Year } 
& 8.62$_{\pm0.09}$ 
& 8.66$_{\pm0.07}$ 
& \textbf{8.56}$_{\pm0.04}$
&-3.59$_{\pm0.08}$
&-3.56$_{\pm0.04}$
&-\textbf{3.51}$_{\pm0.03}$
\\
\bottomrule
\end{tabular}
\end{sc}
\end{table}



\begin{figure}[ht]
    \centering
    \begin{tabular}{cc}
  \includegraphics[width=0.6\textwidth]{figs/MNIST.pdf}  
&
  \includegraphics[width=0.225\textwidth]{figs/MNIST_particle.pdf}  \\
  \includegraphics[trim={7.cm 0.5cm 7cm 0.5cm},clip,width=0.6\textwidth]{figs/legend2.pdf}  &
  \includegraphics[trim={15.cm 0.1cm 15cm 0.1cm},clip,width=0.25\textwidth]{figs/legend3.pdf}  \\
  {\tiny (a) SVGD vs PFG on MNIST classification} & {\tiny(b) PFG with different particles}
    \end{tabular}
    
   % \includegraphics[width=3.5cm]{figs/graph.png}
   
    \caption{
    Test accuracy and NLL of
    Bayesian Neural Network (MNIST classification)
    }%parameterized by $\phi$
    %p_\theta(x,z,u) =
    %induced by $G_\theta^{-1}$
    \label{fig:BNN}
\end{figure}


\noindent \textbf{Time Comparison.} As indicated, our algorithm is more scalable than SVGD in terms of particle numbers.  Tab. \ref{tab:time} shows that SVGD entails more computation cost with the increase of particle numbers. Our functional gradient is obtained with iterative approximation without kernel matrix computation. When $n$ is large, our $O(n)$ algorithm is much faster than $O(n^2)$ kernel-based method. Interestingly, the introduction of particle interactions is a key merit of particle-based VI algorithms, which intuitively needs $O(n^2)$ computation. 
The integration by parts technique draws the connection between the particle interaction and $\nabla\cdot f_\theta$ which supports more efficient computational realizations.

\begin{table}[H]
    \centering
   % \vspace{-0.5cm}
\caption{Time Comparison on Bayesian logistic regression (sonar dataset, 1,000 iterations)}
\vspace{0.2cm}
    \label{tab:time}
    %\small
    \begin{sc}
    \begin{tabular}{c|ccccc}
    \toprule
       \# of particles  &  5 &10 & 100 & 1000 & 2000\\
         \midrule
       SVGD &\textbf{5.20}$_{\pm0.10}$ &\textbf{5.25}$_{\pm0.13}$&\textbf{5.71}$_{\pm0.11}$ & 19.10$_{\pm0.52}$&81.50$_{\pm1.86}$
        \\
        PFG&7.87$_{\pm0.16}$&7.95$_{\pm0.15}$&8.15$_{\pm0.17}$&\textbf{11.56}$_{\pm0.24}$&\textbf{13.22}$_{\pm0.26}$\\
        \bottomrule
    \end{tabular}
        \end{sc}
     %    \vspace{-0.5cm}
\end{table}



%\subsection{Contextual Bandits}




==> parts/method.tex <==
\section{Method}

Given $p_*(x)$, we would like to find $g(t,x)$, so that
starting from $X_0 \sim N(0,I)$, the 
distribution $p(t,x)$ of the following method 
\[
d X_t = g_t(X_t) d t
\]
converges to $p_*(x)$ as $t \to \infty$. 

From the Fokker-Planck equation, we have
\[
\frac{\partial p(t,x)}{\partial t}
= - \nabla \cdot [ g(t,x) p(t,x)]
\]
The KL divergence
\[
KL(t) = \int p(t,x) \ln \frac{p(t,x)}{p_*(x)} dx 
\]
satisfies
\begin{align*}
\frac{d KL(t)}{d t}
=& \int \frac{\partial p(t,x)}{\partial t}
\left(1+ \ln \frac{p(t,x)}{p_*(x)}\right) d x\\
=& - \int  \nabla \cdot [ g(t,x) p(t,x)]
\left(1+ \ln \frac{p(t,x)}{p_*(x)}\right) d x\\
=& \int    [ g(t,x) p(t,x)]^\top
\nabla \ln \frac{p(t,x)}{p_*(x)} d x \\
=& -\int   p(t,x) [\nabla \cdot g(t,x) + g(t,x) p(t,x)
\nabla_x \ln {p_*(x)}] d x .
\end{align*}


We can now let $g(t,x)$ belonging to a vector valued function class $\cF$, and to find the best gradient direction in functional form, we may apply functional form of Frank-Wolfe algorithm:
\[
g(t,x) = \sup_{f \in \cF} 
\int   p(t,x) [\nabla \cdot f(x) + f(x)^\top
\nabla \ln {p_*(x)}] d x .
\]
or gradient boosting:
\[
g(t,x) = \sup_{f \in \cF} \left[
\int   p(t,x) [\nabla \cdot f(x) + f(x)^\top
\nabla \ln {p_*(x)} - \|f(x)\|_2^2\right] d x 
\]
or more generally:
\[
g(t,x) = \sup_{f \in \cF} \left[
\int   p(t,x) [\nabla \cdot f(x) + f(x)^\top
\nabla \ln {p_*(x)} - Q(f)\right] d x ,
\]
where $Q(f)$ is any appropriate regularizer that limits the output magnitude of $f$.

\subsection{Kernel Class}

We assume that 
\[
\cF= \{ W \psi(x), \|W\|_F \leq 1\} ,
\]
and let kernel
\[
k(x,x') = \psi(x)^\top \psi(x') .
\]

The solution  
\[
\hat{W}_t = 
\sup_{\|W\|_F \leq 1} 
\int   p(t,x) \trace[W \nabla \psi(x) + W \psi(x)
\nabla \ln {p_*(x)}^\top] d x 
\]
which gives
\[
\hat{W}_t = 
\int   p(t,x') [\nabla \psi(x')^\top +
\nabla \ln {p_*(x')} \psi(x')^\top] d x' .
\]
This implies that 
\[
g(t,x)=\hat{W}_t \psi(x)
= \int   p(t,x') [\nabla_{x'} k(x',x)+
\nabla \ln {p_*(x')} k(x',x)] d x' 
\]

\subsection{General Model Class}

We can let 
\[
\cF=\{f(\theta,x) \}
\]
and apply gradient boosting or more general formulation as
\[
g(t,x) = 
f(\hat{\theta}_t,x) :
\hat{\theta}_t=\arg\min_\theta \left[
\int   p(t,x) [-\nabla \cdot f(\theta,x) - f(\theta,x)^\top
\nabla \ln {p_*(x)} + 0.5  \|f(\theta,x)-f_0(x)\|_K^2\right] d x 
\]
where we can set
\[
f_0(x)=0
\]
or let 
\[
f_0(x) = -K^{-1} \nabla \ln p_*(x)  ,
\]
where $K$ is some preconditioning matrix.

More generally, we let
\[
g(t,x) = 
f(\hat{\theta}_t,x) :
\hat{\theta}_t=\arg\min_\theta \left[
\int   p(t,x) [-\nabla \cdot f(\theta,x) - f(\theta,x)^\top
\nabla \ln {p_*(x)} \right] d x 
+ Q(\theta) ,
\]
where we can choose 
\[
Q(\theta) = \|\theta-\theta_0\|_K^2 ,
\]
or 
\[
Q(\theta) = h(\theta) - \nabla h(\theta_0)^\top \theta 
\]
for some convex function $h$, 
or
\[
Q(\theta) = \int p(t,x)  
[h(f(\theta,x))-\nabla h(f_0(x))^\top f(\theta,x)] d x
\]
for some convex function $h$. 


